A Bayesian Approach to the Data Description Problem

In this paper, we address the problem of data description using a Bayesian framework. The goal of data description is to draw a boundary around objects of a certain class of interest to discriminate that class from the rest of the feature space. Data description is also known as one-class learning and has a wide range of applications. The proposed approach uses a Bayesian framework to precisely compute the class boundary and therefore can utilize domain information in form of prior knowledge in the framework. It can also operate in the kernel space and therefore recognize arbitrary boundary shapes. Moreover, the proposed method can utilize unlabeled data in order to improve accuracy of discrimination. We evaluate our method using various real-world datasets and compare it with other state of the art approaches of data description. Experiments show promising results and improved performance over other data description and one-class learning algorithms.

==> references.tex <==
%\bibitem{zhou3} Z.-H. Zhou.  {\em Learning with unlabeled data and its application to image retrieval.}  In Proceedings of the 9th Pacific Rim International Conference on Artificial  Intelligence, pages


%\bibitem{docclass} K. Nigam, A. McCallum, and T. Mitchell, {\em Semi-Supervised Text Classification Using EM},  in Semi-Supervised Learning, Olivier Chapelle, Bernhard Scholkopf, and Alexander Zien (eds.), MIT Press, 2006.



%\bibitem{trans} Wei Liu and Shih-Fu Chang,{\em Robust Multi-Class Transductive Learning with Graphs}, IEEE Conference on Computer Vision and Pattern Recognition (CVPR), Miami Beach, Florida, USA, 2009.


%\bibitem{actsvm} Simon Tong, Edward Chang,{\em Support Vector Machine Active Learning for Image Retrieval.}, Proceedings of the ninth ACM international conference on Multimedia, 2001.


%\bibitem{ensmbl} Z-H. Zhou, {\em When semi-supervised learning meets ensemble learning}, in Proc. 8th Int. Workshop, MCS, vol. 4472, Lecture Notes in Computer Science, J. A. Benediktsson, J. Kittler, and F. Roli, Eds., Reykjavik, Iceland, 2009, pp. 529538.


%\bibitem{cosvm} Cheng,  J.,  and  Wang,  K., {\em Active  learning  for image retrieval with Co-SVM.} Pattern Recognition, 40(1), 330-334, 2007.


\bibitem{ocl} D. M. J.  Tax. {\em One-class classification; Concept-learning in the absence of counter-examples.} PhD thesis, Delft University of Technology, 2001.

\bibitem{super} T. Ogawa and M. Haseyama,  \textit{Adaptive Single Image Superresolution Approach Using Support Vector Data Description}. EURASIP J. Adv. Sig. Proc. (EJASP) 2011 (2011).


\bibitem{ocls} S. S. Khan, {\em  A Survey of Recent Trends in One Class Classification.} AICS 2009:188-197.

\bibitem{svdd1} Y. X. DeMenthon and D. S. Doermann, {\em Support Vector Data Description for image categorization from Internet images.} ICPR 2008:1-4.
\bibitem{svdd} D. Tax D. and R. Duin, {\em Support Vector Data Description}, Machine Learning, 54(1):45-66, 2004.

\bibitem{shawe} J. S. Taylor and N. Cristianini, {\em Kernel Methods for Pattern Analysis} Cambridge University Press, 2004.

\bibitem{ddir}  Chen Y.  et. al.,{\em One-class SVM for learning in image retrieval.} ICIP 2001:34-37.
\bibitem{fault}  Y. H. Liu et. al., {\em High-speed inline defect detection for TFT-LCD array process using a novel support vector data description.} Expert Syst. Appl. (ESWA) 38(5):6222-6231 (2011)

\bibitem{bishop2} C. Bishop,{\em Novelty detection and neural network validation.} IEEE Proceedings on Vision, Image and Signal Processing. Special Issue on Applications of Neural Networks 141(4) (1994) 217-222

\bibitem{ocdt} C. Li and Y. Zhang,\textit{ Bagging One-Class Decision Trees}. FSKD 2008:420-423

\bibitem{ocknn1} J. Yang, N. Zhong, P. Liang, J. Wang, Y. Yao and S. Lu, \textit{Brain activation detection by neighborhood one-class SVM}. Cognitive Systems Research (COGSR) 11(1):16-24 (2010)

\bibitem{ocknn2} G. G. Cabral, A. L. I. Oliveira and C. B. G. Cahu, \textit{Combining nearest neighbor data description and structural risk minimization for one-class classification}. Neural Computing and Applications (NCA) 18(2):175-183 (2009)

\bibitem{kde1} G. Cohen, H. Sax and A. Geissbühler, \textit{ Novelty Detection using One-class Parzen Density Estimator. An Application to Surveillance of Nosocomial Infections}. MIE 2008:21-26

\bibitem{kde2} H. Oliveira, J. J. Caeiro and P. L. Correia, \textit{Improved road crack detection based on one-class Parzen density estimation and entropy reduction.} ICIP 2010:2201-2204.

\bibitem{gmm} P. N. Trujillo, P. Drews, R. Rocha, M. F. Montenegro Campos and J. Dias, \textit{Novelty detection and 3D shape retrieval based on Gaussian Mixture Models for autonomous surveillance robotics}. IROS 2009:4724-4730.

\bibitem{svm} C. J. C. Burges, \textit{A Tutorial on Support Vector Machines for Pattern Recognition}. Data Min. Knowl. Discov. (DATAMINE) 2(2):121-167 (1998).

\bibitem{asdd} N. Görnitz, M. Kloft and U. Brefeld,\textit{ Active and Semi-supervised Data Domain Description}. ECML/PKDD 2009:407-422.

\bibitem{ocgp} M. Kemmler, E. Rodner and  J. Denzler: \textit{One-Class Classification with Gaussian Processes}. ACCV 2010:489-500.

\bibitem{bod} J. Ting, A. D'Souza and S. Schaal, \textit{Automatic Outlier Detection: A Bayesian Approach.} ICRA 2007:2489-2494.

\bibitem{bod2} J. M. Coughlan and Alan L. Yuille, \textit{Manhattan World: Orientation and Outlier Detection by Bayesian Inference}. Neural Computation (NECO) 15(5):1063-1088 (2003).

\bibitem{bod4} A. Varbanov, \textit{Bayesian approach to outlier detection in multivariate normal samples and linear models}, Commun. Statist.-Theory Meth. 27 (3), 547-557, 1998.

\bibitem{bod3}  F. Dong, \textit{Bayesian Method to Detect Outliers for Ordinal Data}. Communications in Statistics - Simulation and Computation (CSSC) 39(7):1470-1484 (2010).


\bibitem{lfpso} C. Elkan and K. Noto. {\em Learning classifiers from only positive and unlabelled data.} KDD 2008:213-220. 2008.


%\bibitem{asurv} B. Settles. {\em Active Learning Literature Survey.}Computer Sciences Technical Report 1648, University of Wisconsin-Madison. 2009.

\bibitem{induced} K. Y. Lee, D. Kim, K. H. Lee, D. Lee, \textit{Density-Induced Support Vector Data Description}. IEEE Transactions on Neural Networks (TNN) 18(1):284-289 (2007).


\bibitem{ocsvm} B. Schölkopf, J. C. Platt, J. Shawe-Taylor, A. J. Smola and R. C. Williamson,\textit{ Estimating the Support of a High-Dimensional Distribution}. Neural Computation (NECO) 13(7):1443-1471 (2001).

\bibitem{lfpu} B. Zhang and W. Zuo, {\em  Learning from Positive and Unlabeled Examples: A Survey.} Proceedings of the 2008 International Symposiums on Information Processing (ISIP '08). IEEE Computer Society, Washington, DC, USA, 650-654. 2008.


\bibitem{bishop} C. M. Bishop,{\em  Pattern Recognition and Machine Learning}, Springer, 2006.


%\bibitem{bwest} Jones, M.C.; Marron, J.S.; Sheather, S. J. (1996). { A brief survey of bandwidth selection for density estimation}. Journal of the American Statistical Association 91: 401-407.


%\bibitem{cvrisk} Hall, P.; Marron, J.S.; Park, B.U., {\em Smoothed cross-validation}. Probability Theory and Related Fields 92: 1-20. 1992.


\bibitem{uci} A. Frank and A. Asuncion,{\em  UCI Machine Learning Repository}, [http://archive.ics.uci.edu/ml]. Irvine, CA: University of California, School of Information and Computer Science, 2010.

\bibitem{manning} C. D. Manning P. Raghavan and H. Schütze,{\em  Introduction to Information Retrieval}, Cambridge University Press. 2008.

%\bibitem{aout} Naoki Abe, Bianca Zadrozny, and John Langford. 2006. {\em Outlier detection by active learning.} In Proceedings of the 12th ACM SIGKDD international conference on Knowledge discovery and data mining (KDD '06). ACM, New York, NY, USA, 504-509.

%\bibitem{mise} Wasserman, Larry, {\em All of Nonparametric Statistics}, Springer (2007) 

\bibitem{cedd} S. A. Chatzichristofis and Y. S. Boutalis, {\em  CEDD: Color and Edge Directivity Descriptor: A Compact Descriptor for Image Indexing and Retrieval}, ICVS 2008: 312-322.

\bibitem{caltech} F. Li, R. Fergus and P. Perona, {\em  Learning generative visual models from few training examples: an incremental Bayesian approach tested on 101 object categories.} IEEE. CVPR 2004, Workshop on Generative-Model Based Vision. 2004.

\bibitem{ockernel} P. F. Evangelista, M. J. Embrechts and B. K. Szymanski, \textit{Some Properties of the Gaussian Kernel for One Class Learning}. ICANN 2007:269-278.


\bibitem{surv1} Zhu, X.{\em  Semi-supervised learning with graphs}.   Doctoral dissertation, Carnegie Mellon University. CMU-LTI-05-192, 2005.


\bibitem{surv2} Xiaojin Zhu. {\em  Semi-supervised learning literature survey.} Technical Report 1530, Department of Computer Sciences, University of Wisconsin, Madison, 2005.

\bibitem{casella} G. Casella and R. L. Berger, \textit{Estimation: point and interval.} International Encyclopedia of the Social and Behavioral Sciences, 7, 4744-4749, 2001.

\bibitem{precise} A. Muñoz and J.M. Moguerza,  \textit{One-Class Support Vector Machines and Density Estimation: The Precise Relation}, CIARP 2004:216-223. 

\bibitem{corel} J. Z. Wang, J. Li and G. Wiederhold, \textit{SIMPLIcity: Semantics-Sensitive Integrated Matching for Picture Libraries}. IEEE Trans. Pattern Anal. Mach. Intell. (PAMI) 23(9):947-963 (2001).
